Understanding Behavior of Clinical Models under Domain Shifts

The hypothesis that computational models can be reliable enough to be adopted in prognosis and patient care is revolutionizing healthcare. Deep learning, in particular, has been a game changer in building predictive models, thus leading to community-wide data curation efforts. However, due to inherent variabilities in population characteristics and biological systems, these models are often biased to the training datasets. This can be limiting when models are deployed in new environments, when there are systematic domain shifts not known a priori. In this paper, we propose to emulate a large class of domain shifts, that can occur in clinical settings, with a given dataset, and argue that evaluating the behavior of predictive models in light of those shifts is an effective way to quantify their reliability. More specifically, we develop an approach for building realistic scenarios, based on analysis of \textit{disease landscapes} in multi-label classification. Using the openly available MIMIC-III EHR dataset for phenotyping, for the first time, our work sheds light into data regimes where deep clinical models can fail to generalize. This work emphasizes the need for novel validation mechanisms driven by real-world domain shifts in AI for healthcare.

==> discussion.tex <==
Short section of how we actually made the world better


==> method.tex <==
%A high-level motivation for unsupervised DA and short description of DANN and VADA
In this section, we describe our predictive model and the techniques employed for performing domain adaptation.
% As described earlier, we assumed that we have access to only unlabeled data in the target, and hence we resort to unsupervised domain adaptation.




%%VADA and DANN loss weights???
%
%\noindent \textbf{Domain Adaptation}: The goal of \emph{unsupervised domain adaptation} is to learn a good predictive model for the target domain ($x\sim P_t(x)$) using labeled source examples ($\{(x,y): x\sim P_s(x)\}$) and unlabeled target examples. While subspace alignment strategies have been well studied for domain adaptation, more recently Domain Adversarial Neural Networks (DANN) \cite{ganin2016domain} have become popular. DANN utilizes adversarial training to perform domain alignment, while simultaneously constructing a predictive model in the source domain. In other words, we attempt to learn representations that are domain invariant but can preserve discriminative  properties useful for the predictive modeling. Formally, this can be expressed as:
%\begin{align}
%%\begin{split}
%\min_{\substack{{g\in\mcal{G}, h\in\mcal{H}}\\{f=h\circ g}}} L_y(f; P_s) &+ \lambda_{\mathcal{D}} L_{\mathcal{D}}(g\#P_s, g\#P_t), 
%%\end{split}
%\end{align}where $h$ is the prediction function, $L_y(f; P_s) := \expect_{x,y\sim P_s} [y^\top \ln f(x)]$ is the cross-entropy loss for the labeled source examples, $L_{\mathcal{D}}(\cdot,\cdot)$ is the loss term measuring the distance between the two distributions,
%
%\begin{align}
%\sup_{\mathcal{D}} \expect_{x\sim P_s} \ln \mathcal{D}(g(x)) + \expect_{x\sim P_t} \ln (1-\mathcal{D}(g(x))). \nonumber
%%\end{split}
%\end{align}Here $g$ is a measurable feature generator mapping and $g\#P$ denotes the push-forward of a distribution $P$. This term results in minimizing the variational form of the Jensen-Shannon (JS) divergence \cite{goodfellow2014generative} between source and target feature distributions. While this formulation relies on the assumption that alignment of the domains will enable the use of $h$ for both domains, there is evidence it can fail in practice \cite{shu2018dirt}. Hence, Virtual Adversarial Domain Adaptation (VADA) employs additional regularization in the form of the  conditional entropy $L_{ce}(.; .)$~\cite{shu2018dirt}:
%\begin{align}
%%\begin{split}
%L_{ce}(f; P_t) := -\expect_{x\sim P_t} [f(x)^\top \ln f(x)].
%%\end{split}
%\end{align}Minimizing this cost on the unlabeled target samples pushes the predictor boundaries away from the high density regions. In addition, VADA incorporates virtual adversarial training to ensure that predictions within a neighborhood in the target domain is smooth.
%\begin{align}
%%\begin{split}
%L_{vt}(f; P_t) := \expect_{x\sim P_t} \bigg[\max_{\lVert r\rVert\leq\epsilon} D_{kl} (f(x) \Vert f(x+r)) \bigg] 
%%\end{split}
%\end{align}Hence, the overall objective function of VADA is
%\begin{align}
%%\begin{split}
%\nonumber \min_{\substack{{g\in\mcal{G}, h\in\mcal{H}}\\{f=h\circ g}}} L_y(f; P_s) &+ \lambda_{\mathcal{D}} L_{\mathcal{D}}(g\#P_s, g\#P_t) +\lambda_{s} L_{vt}(f;P_s) \\ &+ \lambda_{t}(L_{ce}(f;P_t)+ L_{vt}(f;P_t)), \nonumber
%%\end{split}
%\end{align}

%\begin{table*}[t]
%	\centering
%	\small
%	\renewcommand{\arraystretch}{1.3}
%	\begin{tabular}{c||c|c|c||c|c|c||c|c|c}
%		\hline
%		& \multicolumn{3}{c||}{\textbf{Source Only}} & \multicolumn{3}{c||}{\textbf{DANN}}                      & \multicolumn{3}{c}{\textbf{VADA}}                      \\
%		\cline{2-10}
%		\multirow{-2}{*}{\textbf{Scenario}}&\textbf{AUROC}     & \textbf{AUPRC}     &\textbf{MCC}     &\textbf{AUROC}         &\textbf{AUPRC}         &\textbf{MCC}           & \textbf{AUROC}         &\textbf{AUPRC}         & \textbf{MCC}           \\
%		\hline
%		\hline
%		\textit{Resp-to-CardiacRenal}             & 0.67      & 0.8       & 0.35    & 0.63          & 0.78          & 0.32          & {0.76} & {0.86} & {0.37} \\
%		\textit{10\% Label Flips}       & 0.73      & 0.83      & 0.33    &  {0.73} &  {0.83} &  {0.38} & 0.65          & 0.78          & 0.31          \\
%		\textit{20\% Label Flips}       & 0.57      & 0.73      & 0.08    & 0.64          & 0.76          & 0.31          &  {0.67} &  {0.88} &  {0.31} \\
%		\textit{Cerebro-to-CardiacRenal}            & 0.63      & 0.82      & 0.26    & {0.69} & {0.85} & {0.26} & 0.65          & 0.81          & 0.26          \\
%		\hline
%		\textit{Older-to-Younger}        & 0.55      & 0.52      & 0.16    &  {0.66} &  {0.64} &  {0.20} & 0.58          & 0.58          & 0.21          \\
%		\textit{Adversarial}        & 0.55      & 0.52      & 0.16    &  {0.62} &  {0.6} &  {0.20} & 0.63          & 0.62          & 0.17          \\
%		\textit{Younger-to-Older}        & 0.6       & 0.9       & 0.1     &  {0.63} &  {0.91} &  {0.12} & 0.61          & 0.9           & 0.11          \\
%		\hline
%		\textit{Male-to-Female}      & 0.68      & 0.67      & 0.23    & 0.64          & 0.67          &  {0.27}          &  {0.68}         &  {0.70}          & 0.25         \\
%		\textit{Female-to-Male}      & 0.68      & 0.85      & 0.22    & 0.66          & 0.84          & 0.23          &  {0.66} &  {0.85} &  {0.24} \\
%		\hline
%		\textit{White-to-Minority}                      &  {0.67}         &  {0.69}         &  {0.25}       & 0.64             & 0.64             & 0.20             & 0.65             & 0.64             & 0.21             \\
%		\hline
%		\textit{Dual-to-Single}            & 0.66      & 0.82      & 0.2     & 0.67          & 0.82          & 0.21          &  {0.67} &  {0.83} &  {0.22} \\
%		\textit{Single-to-Dual}          & 0.8       & 0.78      & 0.39    & 0.81          & 0.8           & 0.51          &  {0.83} &  {0.81} &  {0.5}  \\
%		\hline
%		\textit{Sampling Rate Change}             & 0.74         & 0.84         & 0.34       &  {0.74}             &  {0.84}           &  {0.35}             & 0.73             & 0.84             & 0.33            \\
%		\hline
%		\textit{Missing-Measurements}             &  {0.61}         &  {0.79}         & 0.13       & 0.60            & 0.78           & 0.13             & 0.60             & 0.78             &  {0.14}            \\
%		\hline
%	\end{tabular}
%\end{table*}

==> notation.tex <==
\newcommand{\punt}[1]{}

%%\newtheorem{thm}{Theorem}
\newtheorem{thm}{Theorem}[section]
\newtheorem{theorem}{Theorem}
\newtheorem{lem}{Lemma}[section]
%\newtheorem{claim}[thm]{Claim}
%\newtheorem{cor}[thm]{Corollary}
%\newtheorem{prop}[thm]{Property}
\newtheorem{prop}{Proposition}
\newtheorem{defn}{Definition}[section]
%\theoremstyle{definition}
\newtheorem{condition}{Condition}
%\newtheorem{thm}{Theorem}[section]
\def\argmax{\mathop{\rm arg\,max}}
\def\argmin{\mathop{\rm arg\,min}}
\newcommand{\transpose}{{\scriptscriptstyle T}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\biggram}{\overrightarrow{\mathbf{K}}}
\newcommand{\biggramsep}{{\vK \otimes \vL}}
\newcommand{\veckernel}{\overrightarrow{k}}
\newcommand{\chvec}{\ch_{\veckernel}}
\newcommand{\chvecsep}{\ch_{k\vL}}
\newcommand{\chdict}{\ch_{\cd}}
\newcommand{\expect}{\mathbb{E}}
\newcommand{\integers}{\mathbf{Z}}
\newcommand{\naturals}{\mathbf{N}}
\newcommand{\rationals}{\mathbf{Q}}



\newcommand{\ca}{\mathcal{A}}
\newcommand{\cb}{\mathcal{B}}
\newcommand{\cc}{\mathcal{C}}
\newcommand{\cd}{\mathcal{D}}
\newcommand{\ce}{\mathcal{E}}
\newcommand{\cf}{\mathcal{F}}
\newcommand{\cg}{\mathcal{G}}
\newcommand{\ch}{\mathcal{H}}
\newcommand{\ci}{\mathcal{I}}
\newcommand{\cj}{\mathcal{J}}
\newcommand{\ck}{\mathcal{K}}
\newcommand{\cl}{\mathcal{L}}
\newcommand{\cm}{\mathcal{M}}
\newcommand{\cn}{\mathcal{N}}
\newcommand{\co}{\mathcal{O}}
\newcommand{\cp}{\mathcal{P}}
\newcommand{\cq}{\mathcal{Q}}
\newcommand{\calr}{\mathcal{R}}
\newcommand{\cs}{\mathcal{S}}
\newcommand{\ct}{\mathcal{T}}
\newcommand{\cu}{\mathcal{U}}
\newcommand{\cv}{\mathcal{V}}
\newcommand{\cw}{\mathcal{W}}
\newcommand{\cx}{\mathcal{X}}
\newcommand{\cy}{\mathcal{Y}}
\newcommand{\cz}{\mathcal{Z}}
\newcommand{\cS}{\mathcal{S}}
%\newcommand{\ind}[1]{1(#1)}
%\newcommand{\pr}{P}
\newcommand{\pr}{\mathbb{P}}
\newcommand{\predsp}{\cy}  %{\hat{\cy}}
\newcommand{\outsp}{\cy}

\newcommand{\prxy}{P_{\cx \times \cy}}
\newcommand{\prx}{P_{\cx}}
\newcommand{\prygivenx}{P_{\cy\mid\cx}}
%\newcommand{\ex}{E}
\newcommand{\ex}{\mathbb{E}}
\newcommand{\var}{\textrm{Var}}
\newcommand{\cov}{\textrm{Cov}}
%\newcommand{\sgn}{\textrm{sgn}}
%\newcommand{\sign}{\textrm{sign}}
\newcommand{\kl}{\textrm{KL}}
\newcommand{\law}{\mathcal{L}}
%\newcommand{\eps}{\varepsilon}
\newcommand{\as}{\textrm{ a.s.}}
\newcommand{\io}{\textrm{ i.o.}}
\newcommand{\ev}{\textrm{ ev.}}
\newcommand{\convd}{\stackrel{d}{\to}}
\newcommand{\eqd}{\stackrel{d}{=}}
\newcommand{\del}{\nabla}
\newcommand{\loss}{V}
\newcommand{\risk}{R}
\newcommand{\emprisk}{\hat{R}_{\ell}}
%\newcommand{\lossfnl}{L}
%\newcommand{\emplossfnl}{\hat{L}}
\newcommand{\lossfnl}{\risk}
\newcommand{\emplossfnl}{\emprisk}
\newcommand{\empminimizer}[1]{\hat{#1}_{\ell}} 
\newcommand{\empminimizerfa}{\hat{f}_{\ell}^{1}}
\newcommand{\empminimizerfb}{\hat{f}_{\ell}^{2}}
\newcommand{\minimizer}[1]{#1_{*}} 
\newcommand{\etal}{\textrm{et. al.}}
%\newcommand{\tr}{\operatorname{tr}}
\newcommand{\rademacher}[1]{\calr_{#1}}
\newcommand{\emprademacher}[1]{\hat{\calr}_{#1}}


\newcommand{\trace}{\operatorname{trace}}
%\newcommand{\diag}{\text{diag}}
\newcommand{\rank}{\text{rank}}
\newcommand{\linspan}{\text{span}}
\newcommand{\spn}{\text{span}}
\newcommand{\proj}{\text{Proj}}
%\newcommand{\argmax}{\operatornamewithlimits{arg\,max}}
%\newcommand{\argmin}{\operatornamewithlimits{arg\,min}}
\def\argmax{\mathop{\rm arg\,max}}
\def\argmin{\mathop{\rm arg\,min}}
%\newcommand{\inf}{\operatornamewithlimits{inf}}

\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfl}{\bm{\lambda}}
\newcommand{\bfm}{\mathbf{\mu}}
\newcommand{\vmu}{\bm{\mu}}
\newcommand{\calL}{\mathcal{L}}

%\newcommand{\v0}{\mathbf{0}}
%\newcommand{\v1}{\mathbf{1}}
\newcommand{\vX}{\mathbf{X}}
\newcommand{\vY}{\mathbf{Y}}
\newcommand{\vA}{\mathbf{A}}
\newcommand{\vB}{\mathbf{B}}
\newcommand{\vE}{\mathbf{E}}
\newcommand{\vK}{\mathbf{K}}
\newcommand{\vD}{\mathbf{D}}
\newcommand{\vU}{\mathbf{U}}
\newcommand{\vL}{\mathbf{L}}
\newcommand{\vI}{\mathbf{I}}
\newcommand{\vC}{\mathbf{C}}
\newcommand{\vV}{\mathbf{V}}
\newcommand{\vM}{\mathbf{M}}
\newcommand{\vN}{\mathbf{N}}
\newcommand{\vQ}{\mathbf{Q}}
\newcommand{\vR}{\mathbf{R}}
\newcommand{\vS}{\mathbf{S}}
\newcommand{\vT}{\mathbf{T}}
\newcommand{\vZ}{\mathbf{Z}}
\newcommand{\vW}{\mathbf{W}}
\newcommand{\vH}{\mathbf{H}}
\newcommand{\vsig}{\bm{\Sigma}}
\newcommand{\vSigma}{\bm{\Sigma}}
\newcommand{\vLam}{\bm{\Lambda}}
\newcommand{\vLambda}{\bm{\Lambda}}
\newcommand{\vlam}{\bm{\lambda}}

\newcommand{\vw}{\mathbf{w}}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vxi}{\bm{\xi}}     
\newcommand{\valpha}{\bm{\alpha}}
\newcommand{\vbeta}{\bm{\beta}}
\newcommand{\veta}{\bm{\eta}}
\newcommand{\vsigma}{\bm{\sigma}}
\newcommand{\vepsilon}{\bm{\epsilon}}
\newcommand{\vdelta}{\bm{\delta}}
\newcommand{\vnu}{\bm{\nu}}
\newcommand{\vd}{\mathbf{d}}
\newcommand{\vs}{\mathbf{s}}
\newcommand{\vt}{\mathbf{t}}
\newcommand{\vh}{\mathbf{h}}
\newcommand{\ve}{\mathbf{e}}
\newcommand{\vf}{\mathbf{f}}
\newcommand{\vg}{\mathbf{g}}
\newcommand{\vz}{\mathbf{z}}
\newcommand{\vk}{\mathbf{k}}
\newcommand{\va}{\mathbf{a}}
\newcommand{\vb}{\mathbf{b}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vr}{\mathbf{r}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\vu}{\mathbf{u}}
\newcommand{\vp}{\mathbf{p}}
\newcommand{\vq}{\mathbf{q}}
\newcommand{\vc}{\mathbf{c}}
\newcommand{\vn}{\mathbf{n}}
%\newcommand{\vy}{\boldsymbol{y}}
%\newcommand{\vA}{\boldsymbol{A}}
%\newcommand{\vW}{\mathbf{W}}
\newcommand{\vP}{\mathbf{P}}
\newcommand{\vG}{\mathbf{G}}
%\newcommand{\vH}{\mathbf{H}}
%\def\v{}{\mathbf{{}}}

%%\newcommand{\bold}[1]{\ensuremath{\mathbf{#1}}}

\newcommand{\hil}{\ch}
\newcommand{\rkhs}{\hil}
\newcommand{\manifold}{\cm} 
\newcommand{\cloud}{\cc} 
\newcommand{\graph}{\cg}    
\newcommand{\vertices}{\cv} 
\newcommand{\coreg}{{\scriptscriptstyle \cc}}
\newcommand{\intrinsic}{{\scriptscriptstyle \ci}}
%\newcommand{\intrinsic}{{\ci}}
\newcommand{\ambient}{{\scriptscriptstyle \ca}}
%\newcommand{\isintrinsic}[1]{#1^\text{i}}
\newcommand{\isintrinsic}[1]{#1^{\scriptscriptstyle \ci}}
%\newcommand{\isambient}[1]{#1^\text{a}}
\newcommand{\isambient}[1]{#1^{\scriptscriptstyle \ca}}
\newcommand{\hilamb}{\ch^\ambient}
\newcommand{\hilintr}{\ch^\intrinsic}
\newcommand{\M}{\text{FIX ME NOW}}  %temporary
\newcommand{\ktilde}{\tilde{k}}
\newcommand{\corkhs}{\tilde{\hil}}
\newcommand{\cok}{\ktilde}
\newcommand{\coK}{\tilde{K}}
\newcommand{\copar}{\lambda}
\newcommand{\reg}{\gamma}
\newcommand{\rega}{\gamma_{1}}
\newcommand{\regb}{\gamma_{2}}
\newcommand{\regamb}{\gamma_{\ambient}}
\newcommand{\regintr}{\gamma_{\intrinsic}}
\newcommand{\regfn}{\Omega}
\newcommand{\regfnintr}{\regfn_{\intrinsic}}
\newcommand{\regfnamb}{\regfn_{\ambient}}
\newcommand{\regfncoreg}{\regfn_{\coreg}}
\newcommand{\bq}{\begin{equation}}
\newcommand{\eq}{\end{equation}}
\newcommand{\ba}{\begin{eqnarray}}
\newcommand{\ea}{\end{eqnarray}}

\newcommand{\spana}{\cl^{1}}
\newcommand{\spanb}{\cl^{2}}
\newcommand{\ha}{\hil^{1}}
\newcommand{\hb}{\hil^{2}}
\newcommand{\fa}{f^{1}}
\newcommand{\fb}{f^{2}}
\newcommand{\Fa}{\cf^{1}}
\newcommand{\Fb}{\cf^{2}}
\newcommand{\ka}{k^{1}}
\newcommand{\kb}{k^{2}}
\newcommand{\vcok}{\boldsymbol{\cok}}
\newcommand{\vka}{\vk^{1}}
\newcommand{\vkb}{\vk^{2}}
\newcommand{\Ka}{K^{1}}
\newcommand{\Kb}{K^{2}}
\newcommand{\kux}{\vk_{Ux}}
\newcommand{\kuz}{\vk_{Uz}}
\newcommand{\kuu}{K_{UU}}
\newcommand{\kul}{K_{UL}}
\newcommand{\klu}{K_{LU}}
\newcommand{\kll}{K_{LL}}
\newcommand{\kuxa}{\vk_{Ux}^{1}}
\newcommand{\kuza}{\vk_{Uz}^{1}}
\newcommand{\Kuua}{K_{UU}^{1}}
\newcommand{\Kula}{K_{UL}^{1}}
\newcommand{\Klua}{K_{LU}^{1}}
\newcommand{\Klla}{K_{LL}^{1}}
\newcommand{\kuxb}{\vk_{Ux}^{2}}
\newcommand{\kuzb}{\vk_{Uz}^{2}}
\newcommand{\Kuub}{K_{UU}^{2}}
\newcommand{\Kulb}{K_{UL}^{2}}
\newcommand{\Klub}{K_{LU}^{2}}
\newcommand{\Kllb}{K_{LL}^{2}}

\newcommand{\Ksum}{S}
\newcommand{\ksum}{s}
\newcommand{\vksum}{\vs}

\newcommand{\intrinsicRegMat}{M_{\intrinsic}}
\newcommand{\coregPointCloudMat}{M_{\coreg}}
\newcommand{\vid}[1]{#1^\text{vid}}
\newcommand{\aud}[1]{#1^\text{aud}}
\newcommand{\bad}[1]{#1_\text{bad}}
\newcommand{\empcompat}{\hat{\chi}}

\newcommand{\nn}{\ensuremath{k}}

\newcommand{\uva}{\ushort{\va}}
\newcommand{\uvf}{\ushort{\vf}}
\newcommand{\uvg}{\ushort{\vg}}
\newcommand{\uvk}{\ushort{\vk}}
\newcommand{\uvw}{\ushort{\vw}}
\newcommand{\uvh}{\ushort{\vh}}
\newcommand{\uvbeta}{\ushort{\vbeta}}
\newcommand{\uA}{\ushort{A}}
\newcommand{\uG}{\ushort{G}}

% For Vikas :)
\def\la{{\langle}}
\def\ra{{\rangle}}
\def\R{{\reals}}

%added by AK
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\mbb}[1]{\mathbb{#1}}
\newcommand{\mcal}[1]{\mathcal{#1}}
\newcommand{\remove}[1]{}
\newcommand{\nuc}[1]{\left\lVert #1\right\rVert_*}
\newcommand{\spec}[1]{\left\lVert #1\right\rVert_2}
\newcommand{\frob}[1]{\left\lVert #1\right\rVert_\fro}
\newcommand{\norm}[1]{\left\lVert #1\right\rVert}
\newcommand{\abs}[1]{\left\lvert #1\right\rvert}
\newcommand{\obs}[1]{P_\Omega({#1})}

\newcommand{\red}[1]{{\color{red} #1}}

%\newenvironment{psmallmatrix}{\left(\begin{smallmatrix}} {\end{smallmatrix}\right)}


%%%%%%%%%%%%%%%%%
\newcommand{\ball}{\mathcal{B}}
\newcommand{\sphere}{\mathcal{S}}
%\newcommand{\R}{\mathbb{R}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\domain}{\mathcal{C}}
\newcommand{\polytope}{\mathcal{P}}
\newcommand{\Am}{\bm{A}}
\newcommand{\Bm}{\bm{B}}
\newcommand{\xv}{\bm{x}}
\newcommand{\yv}{\bm{y}}
\newcommand{\zv}{\bm{z}}
\newcommand{\sv}{\bm{s}}
\newcommand{\av}{\bm{a}}
\newcommand{\bv}{\bm{b}}
%\newcommand{\cv}{\bm{c}}
%\newcommand{\ev}{\bm{e}}
\newcommand{\pv}{\bm{p}}
\newcommand{\uv}{\bm{u}}
%\newcommand{\vv}{\bm{v}}
\newcommand{\wv}{\bm{w}}
\newcommand{\omegav}{\bm{\omega}}
\newcommand{\mv}{\bm{m}}
\newcommand{\GW}{G_\setC}%{G_{\!f,\setC}}
\newcommand{\G}{G}
\newcommand{\0}{\bm{0}}
\newcommand{\id}{\bm{\iota}}
\newcommand{\alphav}{\bm{\alpha}}
\newcommand{\nuv}{\bm{\nu}}
\newcommand{\thetav}{\bm{\theta}}
\newcommand{\lambdav}{\bm{\lambda}}
\newcommand{\epsilonv}{\bm{\epsilon}}
%\newcommand{\GW}{gap_{FW}}
\newcommand{\row}{\text{row}}
\newcommand{\col}{\text{col}}
\newcommand{\lft}{\text{left}}
\newcommand{\rgt}{\text{right}}
\newcommand{\one}{\mathbf{1}} % all one vector




\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\dom}{dom}         % domain

\newcommand{\todo}[1]{\marginpar[\hspace*{4.5em}\textbf{TODO}\hspace*{-4.5em}]{\textbf{TODO}}\textbf{TODO:} #1}


\newcommand{\aatop}[2]{\genfrac{}{}{0pt}{}{#1}{#2}}
%\newcommand{\etal}{\textit{et al}.}
\newcommand{\ie}{\textit{i}.\textit{e}.}
\newcommand{\eg}{\textit{e}.\textit{g}.}

\newcommand{\blue}[1]{\textcolor{blue}{#1}}

